Subexponential parameterized algorithms for planar and apex-minor-free graphs via low treewidth pattern covering

We prove the following theorem. Given a planar graph $G$ and an integer $k$, it is possible in polynomial time to randomly sample a subset $A$ of vertices of $G$ with the following properties: (i) $A$ induces a subgraph of $G$ of treewidth $\mathcal{O}(\sqrt{k}\log k)$, and (ii) for every connected subgraph $H$ of $G$ on at most $k$ vertices, the probability that $A$ covers the whole vertex set of $H$ is at least $(2^{\mathcal{O}(\sqrt{k}\log^2 k)}\cdot n^{\mathcal{O}(1)})^{-1}$, where $n$ is the number of vertices of $G$. Together with standard dynamic programming techniques for graphs of bounded treewidth, this result gives a versatile technique for obtaining (randomized) subexponential parameterized algorithms for problems on planar graphs, usually with running time bound $2^{\mathcal{O}(\sqrt{k} \log^2 k)} n^{\mathcal{O}(1)}$. The technique can be applied to problems expressible as searching for a small, connected pattern with a prescribed property in a large host graph, examples of such problems include Directed $k$-Path, Weighted $k$-Path, Vertex Cover Local Search, and Subgraph Isomorphism, among others. Up to this point, it was open whether these problems can be solved in subexponential parameterized time on planar graphs, because they are not amenable to the classic technique of bidimensionality. Furthermore, all our results hold in fact on any class of graphs that exclude a fixed apex graph as a minor, in particular on graphs embeddable in any fixed surface.

==> applications.tex <==
\section{Applications}\label{sec:applications}

==> clustering.tex <==
\section{Clustering tools}\label{sec:clustering}

\begin{comment}
In this section we develop two algorithms --- one randomized and one deterministic --- dubbed \emph{clustering tools}.
The goal of the randomized algorithm is to delete some vertices of the graph so that every connected component of the remaining graph has small radius and, at the same time, the probability of spoiling 
the sought pattern is also small. We aim at small being (inverse-)polynomial in $k$ and $\log n$.

We start with a simple randomized procedure that we do not know how to derandomize.
Then, we develop a more involved deterministic procedure that will work only for graphs with a fixed excluded minor.

\subsection{Simple randomized procedure}
\end{comment}

\begin{theorem}\label{thm:clust}
There exists a randomized polynomial-time algorithm that, given a graph $G$ on $n>1$ vertices and a positive integer $k$, returns a vertex subset $B\subseteq V(G)$ with the following properties:
\begin{enumerate}[(a)]
\item The radius of each connected component of $G[B]$ is less than $9k^2\lg n$.
\item For each vertex subset $X\subseteq V(G)$ of size at most $k$, the probability that $X \subseteq B$ is at least $1-\frac{1}{k}$.
\end{enumerate}
\end{theorem}
\begin{proof}
Consider the following iterative procedure which constructs a set $B_0$. We start with $V_0 = V(G)$.
In the step $i$, given a set $V_{i-1} \subseteq V(G)$, we terminate the procedure if $V_{i-1} = \emptyset$.
Otherwise we pick an arbitrary vertex $v_i \in V_{i-1}$ and we randomly select a radius $r_i$ according to the geometric distribution with success probability $p := \frac{1}{2k^2}$.
Given $v_i$ and $r_i$, we insert $\distball_{G[V_{i-1}]}(v_i,r_i-1)$ into $B_0$ and define $V_i := V_{i-1} \setminus \distball_{G[V_{i-1}]}(v_i,r_i)$.
That is, we delete from the graph vertices within distance at most $r_i$ from $v_i$ in $G[V_{i-1}]$, and put the vertices within distance \emph{less} than $r_i$ into $B_0$.
Finally, at the end of the procedure, if any of the selected radii $r_i$ is larger than $9k^2 \lg n$, we return $B = \emptyset$, and otherwise we return $B=B_0$.

Clearly, the procedure runs in polynomial time, as at every step at least the vertex $v_i$ is removed from $V_{i-1}$, and hence at most $n$ iterations are executed.
For the radii of the connected components of $G[B_0]$, note that the fact that we insert into $B_0$ vertices within distance \emph{less} than $r_i$ from $v_i$, but delete
from $V_i$ vertices within distance \emph{at most} $r_i$ from $v_i$, ensures that at every step $i$ of the iteration we have $N_G[B_0] \cap V_i = \emptyset$. Consequently,
$\distball_{G[V_{i-1}]}(v_i,r_i-1)$ induces a connected component of $G[B_0]$, and is of radius less than $r_i$. 
Since we return $B = \emptyset$ instead of $B=B_0$ if any of the selected radii $r_i$ exceeds $9k^2 \lg n$, the upper bound on the radii of the connected components of $G[B]$ follows.

It remains to argue that any fixed $k$-vertex subset $X \subseteq V(G)$ survives in $B$ with high probability. 
First, note that for fixed $i$ we have that 
$$\mathbb{P}(r_i > 9k^2 \lg n) \leq \left(1-p\right)^{9k^2 \lg n} \leq e^{-4.5 \lg n} < n^{-3} < \frac{1}{2kn};$$
here, we use the fact that $p=\frac{1}{2k^2}$ and the inequality $1-x\leq e^{-x}$.
Thus, as there are at most $n$ iterations, with probability less than $\frac{1}{2k}$ the algorithm returns $B = \emptyset$ because of some $r_i$ exceeding the limit of $9k^2 \lg n$.

Second, we analyse the probability that $X\subseteq B_0$. Let us fix some $x \in X$.
The only moment where the vertex $x$ could be deleted from the graph, but not put into $B_0$, is when $x$ is within distance exactly $r_i$ from the vertex $v_i$ in an iteration $i$.
It is now useful to think of the choice of $r_i$ in the iteration $i$ as follows: we start with $r_i := 1$ and then, iteratively, with probability $p$ accept the current radius,
and with probability $1-p$ increase the radius $r_i$ by one and repeat.
However, in the aforementioned interpretation of the geometric distribution, when $r_i = \distance_{G[V_{i-1}]}(v_i,x)$, with probability $p$ the radius $r_i$ is accepted
(and $x$ is deleted but not put in $B_0$), but with probability $(1-p)$ the radius $r_i$ is increased, and the vertex $x$ is included in the ball
$\distball_{G[V_{i-1}]}(v_i,r_i-1) \subseteq B_0$. Consequently, the probability that a fixed vertex $x \in X$ is not put into $B_0$ is at most $p$.
By the union bound, we infer that the probability that $X \not\subseteq B_0$ is at most $kp = \frac{1}{2k}$. Together with the $\frac{1}{2k}$ upper bound on the probability
that the maximum radius among $r_i$ exceeds $9k^2\lg n$, which results in putting $B=\emptyset$ instead of $B=B_0$, we have that the probability that $X\not\subseteq B$ is at most $\frac{1}{k}$.
This concludes the proof.
\end{proof}
\begin{comment}

\subsection{Deterministic procedure}

The drawback of the algorithm of Theorem~\ref{thm:clust} is that we do not know how to derandomize it. 
Now we develop a more involved procedure, relying on sparsity, that is deterministic.

\begin{definition}
For an $n$-vertex graph $G$ and an integer $k$, a family $\mathcal{B}$ of subsets of $V(G)$ is called a \emph{covering family of radius $r$ and size $s$}
if
\begin{description}
\item[(covering property)] for every $X \subseteq V(G)$ of size at most $k$, there exists $B \in \mathcal{B}$ with $X \subseteq B$;
\item[(radius bound)] for every $B \in \mathcal{B}$, the radius of every connected component of $G[B]$ is at most $r$; and
\item[(size bound)] $|\mathcal{B}| \leq s$.
\end{description}
\end{definition}
A small covering family of bounded radius is the deterministic analog of the randomized procedure of Theorem~\ref{thm:clust}.
In what follows, we aim at at the radius and size bounds polynomial in $k$ and $\log n$.

We start with graphs of bounded treewidth.
\begin{theorem}\label{thm:clust-tw}
Given a graph $G$, an integer $k$, and a tree decomposition of $G$ of width at most $t$,
one can in polynomial time compute a covering family of $G$ of radius and size $\Oh(kt \log n)$.
\end{theorem}

\begin{proof}
We construct a set $B_r$ for every integer $1 \leq r \leq M$ for $M := k(t+1)\lceil \log (n+1) \rceil + 1$, and define $\mathcal{B} = \{B_r : 1 \leq r \leq M\}$.

Let us fix an integer $r$ as above, and invoke the following recursive procedure for every connected component $G'$ of $G$.
At every recursive step, $G'$ will be an induced subgraph of $G$; thus, the input tree decomposition naturally induces a tree decomposition of $G'$ of width at most $t$.
Consequently, we can find a set $Z \subseteq V(G')$ of size at most $t+1$ such that every connected component of $G'-Z$ has at most $|V(G')|/2$ vertices.
Sequentially, for every $z \in Z$, we insert $\distball_{G'}(z,r-1)$ into $B_r$ and remove $\distball_{G'}(z,r)$ from $G'$.
Finally, we recurse on every connected component of the remaining graph $G'$.

Since at every step we remove from $G'$ all vertices within distance at most $r$ from $z$, but insert into $B_r$ all vertices within distance less than $r$ from $z$, we maintain
an invariant that $N_G[B_r] \cap V(G') = \emptyset$ and, consequently, the inserted sets $\distball_{G'}(z,r-1)$ are exactly the vertex sets of the connected components of $G[B_r]$.
Hence, every connected component of $G[B_r]$ is of radius less than $r = \Oh(kt \log n)$.

Consider now a vertex $x \in V(G')$, and consider a single step of the recursive procedure. Given the radius $r$, the vertex $x$ either
\begin{enumerate}[(i)]
\item is removed from $G'$ and inserted into $B_r$; 
\item is removed from $G'$ but not inserted into $B_r$; or 
\item remains in a connected component of $G'$.
\end{enumerate}
Since every vertex in $Z$ is removed from $G'$, in the last case the size of the connected component that contains $x$ drops by at least a half. Consequently,
every vertex $x \in V(G)$ is contained in a graph $G'$ considered by the recursive procedure at most $\lceil \log (n+1) \rceil$ times.

Assume for a moment that the parameter $r$ is chosen randomly, uniformly at random from the set $\{1,2,\ldots,M\}$.
For a fixed step of the recursive procedure on a graph $G'$, for a fixed $z \in Z$, the probability that $r = \distance_{G'}(x,z)$ is $1/M$. Since $|Z| \leq t+1$,
the probability that option (ii) happens for a fixed vertex $x \in V(G)$ is at most $\frac{t+1}{M}$. Since $x$ is contained in a graph $G'$ considered by the recursive procedure
at most $\lceil \log(n+1) \rceil$ times, we have that the probability that a fixed vertex $x \in V(G)$ is not included in $B_r$ is at most $\frac{(t+1)\lceil \log(n+1) \rceil}{M}$.\
By union bound, the probability that a fixed set $X$ of at most $k$ vertices is not contained in $B_r$ is at most $\frac{k(t+1)\lceil \log(n+1) \rceil}{M} = \frac{M-1}{M} < 1$.
Hence, for at least one integer $1 \leq r \leq M$, the set $B_r$ contains $X$. This concludes the construction
of the family $\mathcal{B}$.
\end{proof}

From the bounded treewidth case, the following excluded-minor case follows easily by the application of the generalization
of the Baker's shifting technique.
\begin{theorem}\label{thm:clust-det}
For every proper minor-closed graph class, given a graph $G$ from this class and an integer $k$,
one can in polynomial time compute a covering family of $G$ of radius $\Oh(k^2 \log n)$ and size $\Oh(k^3 \log n)$.
\end{theorem}
\begin{proof}
We apply the algorithm of~\cite[Theorem 3.1]{DemaineHK05} that,
in polynomial time, partitions $V(G)$ into $k+1$ parts $P_1,P_2,\ldots,P_{k+1}$, such that $G-P_i$ is of treewidth $\Oh(k)$ for every $1 \leq i \leq k+1$
(note that the constant hidden here in the big-$\Oh$ notation depends on the graph class).
For every part $P_i$, we first compute a tree decomposition of $G-P_i$ of width $\Oh(k)$ using the constant-approximation
algorithm for graphs excluding a fixed minor of~\cite{FeigeHL08}, and then we apply Theorem~\ref{thm:clust-tw} to the graph $G-P_i$ with the constructed tree decomposition,
obtaining a family $\mathcal{B}_i$ of radius and size $\Oh(k^2 \log n)$.
We output $\mathcal{B} := \bigcup_{1 \leq i \leq k+1} \mathcal{B}_i$. Clearly, $\mathcal{B}$ satisfies the claimed radius and size bounds.
For the covering property, note that for every $X \subseteq V(G)$ of size at most $k$, there exists $i$ such that $X \cap P_i = \emptyset$,
and, consequently, $X \subseteq B$ for some $B \in \mathcal{B}_i$.
\end{proof}
\end{comment}
